Text-Only Training for Image Captioning using Noise-Injected CLIP

We consider the task of image-captioning using only the CLIP model and additional text data at training time, and no additional captioned images. Our approach relies on the fact that CLIP is trained to make visual and textual embeddings similar. Therefore, we only need to learn how to translate CLIP textual embeddings back into text, and we can learn how to do this by learning a decoder for the frozen CLIP text encoder using only text. We argue that this intuition is "almost correct" because of a gap between the embedding spaces, and propose to rectify this via noise injection during training. We demonstrate the effectiveness of our approach by showing SOTA zero-shot image captioning across four benchmarks, including style transfer. Code, data, and models are available on GitHub.

==> tables/tab.tex <==




\begin{table*}
\footnotesize
\begin{center}

$(A)$ \textbf{Conceptual Captions}
\begin{tabular}{p{0.17\textwidth}ccccc}
\toprule
Model &  ROUGE-L $\uparrow$ & CIDEr $\uparrow$ & SPICE $\uparrow$ & \#Params (M) $\downarrow$ & Training Time  $\downarrow$ \\ 
\bottomrule
\midrule
VLP & $24.35$ & $ 77.57$ & $16.59$ & 115 & $ 1200$h (V$100$)\\
\toprule
Ours; MLP + GPT2 tuning & $\mathbf{26.71}$ & $\mathbf{87.26}$ & $\mathbf{18.5}$ & $156$ & $80$h (GTX$1080$)\\
\midrule
% Ours w/ beam search & $26.51$ & $89.58$ & $18.2$ & 31 & $ 168$ (GTX$1080$)\\
% \midrule
Ours; Transformer & $25.12$ & $71.82$ & $16.07$ & $\mathbf{43}$ & $
\mathbf{72}$\textbf{h} (GTX$1080$) \\
\bottomrule 
\end{tabular}
% {'Bleu_1': 0.24489445029532422, 'Bleu_2': 0.1429134077174941, 'Bleu_3': 0.09088275309299156, 'Bleu_4': 0.060227730730366164, 'METEOR': 0.10208756150946528, 'ROUGE_L': 0.24821681573999405, 'CIDEr': 0.7063327299389974, 'SPICE': 0.16029866781695395}
\vspace{0.15cm}

$(B)$ \textbf{nocaps}


\begin{tabular}{l|cc|cc|cc|cc|cc}
\toprule

& \multicolumn{2}{c}{in-domain} & \multicolumn{2}{c}{near-domain} & \multicolumn{2}{c}{out-of-domain} & \multicolumn{2}{c}{Overall} & & \\
Model &  CIDEr  & SPICE   & CIDEr & SPICE & CIDEr & SPICE & CIDEr & SPICE & Params & Time  \\ 
\bottomrule
\midrule
BUTD ~\cite{anderson2018bottom}  & $74.3$ & $ 11.5$ & $56.9$ & $10.3$ & $30.1$ & $8.1$ & $ 54.3$ & $10.1$ & $52$ & $960$h  \\
\midrule
Oscar ~\cite{li2020oscar} & $79.6$ & $ \mathbf{12.3}$ & $66.1$ & $\mathbf{11.5}$ & $45.3$ & $\mathbf{9.7}$ & $ 63.8$ & $\mathbf{11.2}$ & $135$ & $74$h\\
\toprule
Ours; MLP + GPT2 tuning & $79.73$ & $ 12.2$ & $\mathbf{67.69}$ & $11.26$ & $\mathbf{49.35}$ & $ \mathbf{9.7}$ & $ 65.7$ & $11.1$& $156$ & $7$h\\
\midrule
Ours; Transformer & $\mathbf{84.85}$ & $ 12.14$ & $66.82$ & $10.92$ & $49.14$ & $9.57$ & $ \mathbf{65.83}$ & $10.86$ &$\mathbf{43}$ & $\mathbf{6}$\textbf{h} \\
% \midrule
% Ours & $26.71$ & $87.26$ & $18.5$ & 31 & $ 168$ (GTX$1080$)\\
% \midrule
\midrule
\end{tabular}

\vspace{0.15cm}
$(C)$ \textbf{COCO}


\begin{tabular}{lcccccc}
\toprule
Model &   B@$4\uparrow$  & METEOR $\uparrow$ & CIDEr $\uparrow$ & SPICE $\uparrow$ & \#Params (M) $\downarrow$ & Training Time $\downarrow$ \\ 
\bottomrule
\midrule
BUTD ~\cite{anderson2018bottom} &  $36.2$ & $27.0$ & $113.5$ & $20.3$ & 52 & $960$h (M$40$)\\
\midrule
VLP ~\cite{zhou2020unified} &  $36.5$ & $28.4$ & $117.7$ & $21.3$ & 115 & $48$h (V$100$)\\
\midrule
Oscar ~\cite{li2020oscar} & $\mathbf{36.58}$ & $\mathbf{30.4}$ &  $\mathbf{124.12}$ & $\mathbf{23.17}$ &  $135$ & $74$h (V$100$)\\

\toprule
Ours; Transformer   & $33.53$ & $27.45$ &  $113.08$ & $21.05$ & $\mathbf{43}$ & $\mathbf{6}$\textbf{h} (GTX$1080$)\\
\midrule

Ours; MLP + GPT2 tuning & $32.15$ & $27.1$ &  $108.35$ & $20.12$ & $156$ & $7$h (GTX$1080$)\\

\midrule

\multicolumn{7}{c}{$(D)$ \textbf{Ablation}} \\
\bottomrule
\midrule

Ours; Transformer + GPT2 tuning  & $32.22$ & $27.79$ &  $109.83$ & $20.63$ & $167$ & $7$h (GTX$1080$) \\

\midrule
Ours; MLP & $27.39$ & $24.4$ & $92.38$ & $18.04$ & $32$ & $6$h (GTX$1080$)\\
\midrule

\end{tabular}


\end{center}
\vspace{-0.1cm}
\caption{Quantitative evaluation. As can be seen, our method achieves comparable results for both nocaps and Conceptual Captions with much faster training time. %*Training time of VLP and Oscar does not include pre-training
}
%\vspace{-0.3cm}
\label{tab:num} 
\end{table*}

==> tables/table2.tex <==
\begin{tabular}{lccccccccccc}
    \toprule
    \multirow{2}{50pt}{\textbf{Model}} &
    \multicolumn{5}{c}{MS-COCO $\Longrightarrow$ Flickr30k} &
    \multicolumn{5}{c}{Flickr30k $\Longrightarrow$ MS-COCO} \\
    \cmidrule(lr){2-6} \cmidrule(lr){7-11} &
    B@1 & B@4 & M & R-L & CIDEr & 
    B@1 & B@4 & M & R-L & CIDEr  \\
    \midrule
    Top-$k$ & 34.9 & 2.4 & 7.5 & 24.2 & 2.3 & 30.0 & 1.8 & 8.5 & 23.6 & 2.5 \\
    Nucleus & 33.4 & 1.7 & 7.0 & 23.3 & 1.8 & 29.1 & 1.6 & 8.0 & 22.9 & 2.1 \\
    Contrastive & 40.3 & 5.3 & 10.7 & 30.5 & 5.1 & 33.8 & 3.2 & 10.2 & 25.5 & 4.2 \\
    CLIPRe & 38.7 & 4.4 & 9.6 & 27.2 & 5.9 & 31.1 & 3.0 & 9.9 & 22.8 & 8.5 \\
    MAGIC & 46.4 & 6.2 & 12.2 & 31.3 & 17.5
    & 41.4 & 5.2 & 12.5 & 30.7 & 18.3 \\
    \midrule
    
    \textbf{ClipL2V} & \textbf{60.2} & \textbf{17.3} & \textbf{18.6} & \textbf{42.7} & \textbf{35.7}
    & \textbf{43.3} & \textbf{9.2} & \textbf{16.3} & \textbf{36.7} & \textbf{27.3} \\
    
    \toprule
\end{tabular}

